Forensic Self-Descriptions Are All You Need for Zero-Shot Detection, Open-Set Source Attribution, and Clustering of AI-generated Images

The emergence of advanced AI-based tools to generate realistic images poses significant challenges for forensic detection and source attribution, especially as new generative techniques appear rapidly. Traditional methods often fail to generalize to unseen generators due to reliance on features specific to known sources during training. To address this problem, we propose a novel approach that explicitly models forensic microstructures - subtle, pixel-level patterns unique to the image creation process. Using only real images in a self-supervised manner, we learn a set of diverse predictive filters to extract residuals that capture different aspects of these microstructures. By jointly modeling these residuals across multiple scales, we obtain a compact model whose parameters constitute a unique forensic self-description for each image. This self-description enables us to perform zero-shot detection of synthetic images, open-set source attribution of images, and clustering based on source without prior knowledge. Extensive experiments demonstrate that our method achieves superior accuracy and adaptability compared to competing techniques, advancing the state of the art in synthetic media forensics.

==> figures/JpegRobustnessViz.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/jpeg_robustness}
    \caption{Our method's zero-shot detection performance vs. different JPEG quality factors}
    \label{fig:jpeg_robustness}
\end{figure}

==> sections/Abstract_v0.tex <==
\begin{abstract}
	
\vspace{-1em}

The rapid evolution of AI-generated image synthesis presents a significant challenge in identifying manipulated or synthetic media, especially when new generative models emerge that differ fundamentally from those previously encountered. In this paper, we propose a novel zero-shot, unsupervised method for detecting AI-generated images based on the concept of forensic self-description. Leveraging insights from multimedia forensics, we extract forensic microstructures—statistical correlations between adjacent pixel values—through a self-supervised learning process applied solely to real images. These microstructures are then used to build a forensic self-descriptive model for each image, capturing intrinsic properties of its creation process. Our extensive experiments demonstrate that this approach achieves near-perfect accuracy in distinguishing AI-generated images from real ones, regardless of the training dataset used. Additionally, our method facilitates source attribution and open-set detection through unsupervised clustering, providing a promising solution for tackling the growing challenge of AI-generated media detection in diverse and evolving scenarios.

\end{abstract}

==> sections/Abstract_v1.tex <==



\begin{abstract}


The emergence of sophisticated AI-generated images poses significant challenges for forensic detection and source attribution, especially as new generative techniques appear rapidly. Traditional methods often fail to generalize to unseen generators due to reliance on features specific to known sources during training. To address this problem, we propose a novel approach that explicitly models forensic microstructures—subtle, pixel-level patterns unique to the image creation process. By learning diverse predictive filters in a self-supervised manner using only real images, we extract residuals that capture different aspects of these microstructures. Jointly modeling these residuals across multiple scales yields a compact parametric model, whose parameters constitute a unique forensic self-description for each image. This self-description enables zero-shot detection of synthetic images without prior exposure, open-set attribution to source generators, and clustering of images based on their sources without any prior knowledge. Extensive experiments demonstrate our method's superior accuracy and adaptability compared to conventional techniques, advancing synthetic media forensics.

\end{abstract}
\vspace{-1.6em}





==> sections/ApplicationClustering_v0.tex <==
\subsection{Unsupervised Clustering of Image Sources}
\label{sec:application_clustering}

In forensic investigations, analysts may encounter collections of images from unlabelled sources. Organizing these images according to their sources without prior knowledge is an important but understudied problem. Unsupervised clustering of image sources facilitates the exploration and organization of such datasets and can help in identifying new and emerging generative sources.

The forensic self-descriptions enable clustering by first extracting the these descriptions for all images in a dataset. We can then simply apply a clustering algorithm like K-means directly on these descriptions to group images based on the their similarity or closeness. The number of clusters can be chosen based on prior knowledge of the expected number of sources or determined using techniques such as the elbow method or silhouette analysis.


% The forensic self-descriptions derived from our method not only enable detection and attribution tasks but also facilitate unsupervised clustering of images based on their sources. 
% Given that the forensic self-descriptions capture intrinsic forensic microstructures unique to each image source, images originating from the same source will have forensic self-description embeddings clustered close together, while images from different sources are expected to have embeddings that are further apart. Therefore, we can group a large set of unlabelled images into clusters that reflect their source identities.
% This capability is particularly valuable for organizing and understanding large collections of images without any labels, allowing for the discovery of underlying patterns and relationships among different image sources, including both real and synthetic origins.


% To achieve this, we first extract the forensic self-description embeddings for all images in our dataset, which may include real images and images generated by various AI-generators. We then apply K-Means clustering directly on these embeddings. The number of clusters can be chosen based on prior knowledge of the expected number of sources or determined using techniques such as the elbow method or silhouette analysis. We will show later in our experimental evaluation that our approach simplifies the clustering process and provides a powerful tool for exploring and organizing large collections of images based on their sources.










==> sections/ApplicationOpenSet_v0.tex <==
\subsection{Open-Set Synthetic Image Source Attribution}
\label{sec:application_openset}

Accurately attributing an image to its source—whether real or from a specific synthetic generator—is another critical forensic task. This becomes particularly challenging when images originate from a generator not encountered during training. Open-set source attribution addresses this by allowing for the possibility that an image comes from an unknown source, unlike closed-set approaches that force attribution to known sources.

Using the self-description of forensic microstructures, open-set source attribution can be performed by first collecting a set of images generated by each generator. Then, for a set of images from each generator, we model the distribution of their corresponding embeddings using a GMM: $p(\phi | S) = = \sum_{\ell}\pi_\ell \mathcal{N}(\boldsymbol{\mu}_\ell, \boldsymbol{\Sigma}_\ell)$, where $S$ is a source of an image. This will result in one GMM for each known generator source. After training the GMMs, we can then use them to attribute the source of a test image by  computing the likelihood of its embedding under each GMM. The generator source with the highest likelihood is considered to be the candidate source of the image: 
\begin{equation}
    S^* = \arg\max_{S} p(\phi | S)
\end{equation}
And if $p(\phi | S^*) < \tau_{\text{reject}}$, the image is considered to be from an unknown source, otherwise, the candidate source is accepted.


% The forensic self-description can not only be used to distinguish between real and AI-generated images, but also be leveraged for open-set source attribution of AI-generator algorithms. This is possible because prior research has shown that differences in the architecture of the generative models result in unique forensic microstructures that can be learned and exploited for source attribution. As we will show later in our experiments, these differences manifest in the forensic self-descriptions of images generated by different AI-generators. This allows us to not only accurately attribute images to a set of known AI-generators, but also to detect images generated by unseen AI-generators.

% To do this, for a given set of known generators, we first collect a set of images generated by each generator. We then extract the forensic self-description embeddings of these images using the proposed method. Then, for a set of images from each generator, we model the distribution of their corresponding embeddings using a GMM. This will result in one GMM for each known generator source. After training the GMMs, we can then use them to attribute the source of a test image by extracting its embedding and computing the likelihood of this embedding under each GMM. The generator source with the highest likelihood that exceeds a predefined rejection threshold is considered the source of the image. If the highest likelihood is below this rejection threshold, the image is considered to be generated by an unknown AI-generator. 










==> sections/ApplicationZeroShot_v0.tex <==
\subsection{Zero-Shot Synthetic Image Detection}
\label{sec:application_zeroshot}

In this paper, zero-shot detection refers to the task of determining whether an image is real or AI-generated without prior exposure to images from the generator in question. Traditional detectors often struggle in this scenario because they rely on feature representations optimized to discriminate between real images and those from known generators.

Most existing detectors learn embeddings that capture aspects of forensic microstructures highly discriminative for the training set but may overlook features pertinent to unseen generators. Consequently, they may fail to detect images from new sources due to the absence of relevant microstructural information in their learned representations.

In contrast, the self-description of an image's forensic microstructures is obtained in a self-supervised manner, capturing all elements of these microstructures—not just those useful for discriminating among known sources. This comprehensive representation allows for building a model of the microstructures present in real images. By performing out-of-distribution detection, images whose microstructures deviate significantly from those of real images can be identified as AI-generated.

This approach can be implemented simply by training a Gaussian Mixture Model (GMM) exclusively on the forensic self-descriptions of real images. During inference, the likelihood of a test image's self-description under the trained GMM is computed: $p(\phi | \text{Real}) = \sum_{\ell}\pi_\ell \mathcal{N}(\boldsymbol{\mu}_\ell, \boldsymbol{\Sigma}_\ell)$, where $\pi_\ell$, $\boldsymbol{\mu}_\ell$, and $\boldsymbol{\Sigma}_\ell$ are the mixing coefficients, means, and covariances of the GMM components, respectively. The test image is classified as real if $p(\phi | \text{real}) \geq \tau_{\text{real}}$ and synthetic otherwise.

%To do this, we first extract the forensic self-descriptions embedding for a set of training real images using our proposed method. Then, we model the distribution of these embeddings originating from real images only using a Gaussian Mixture Model (GMM). After training the GMM, we can classify a test image as real or synthetic based on the likelihood of its embedding under the trained GMM.


\begin{comment}
# Applications

## 1. Zero-Shot Synthetic Image Detection

In this section, we demonstrate how the forensic self-descriptions derived from individual images enable effective zero-shot detection of synthetic images. Leveraging the significant differences in forensic microstructures between real and AI-generated images, we frame the detection task as an out-of-distribution problem. By modeling the distribution of forensic self-descriptions from real images, we can identify synthetic images as outliers without prior exposure to specific generative models.

### 1.1. Background and Motivation

As established in prior research, real images captured by cameras exhibit forensic microstructures that differ markedly from those in AI-generated images. These differences arise due to the complex imaging pipeline in cameras, including sensor characteristics, demosaicing algorithms, and compression artifacts, which collectively leave distinctive traces in the image. In contrast, synthetic images generated by AI algorithms lack these specific traces or exhibit alternative artifacts introduced by generative models.

Our forensic self-description embeddings capture these intrinsic properties by modeling the forensic residuals of each image. Consequently, embeddings from real images are expected to cluster together in the feature space, while those from synthetic images will deviate from this distribution. This observation motivates the use of out-of-distribution detection techniques to identify synthetic images.

### 1.2. Detection Methodology

#### 1.2.1. Forensic Self-Description Embeddings

From our proposed method, each image \( I \) yields a forensic self-description embedding \( \mathbf{f} \in \mathbb{R}^d \), obtained by flattening the optimized parameters \( \mathbf{W}_\eta^* \):

\[
\mathbf{f} = \text{vec}\left( \mathbf{W}_\eta^* \right).
\]

These embeddings encapsulate the unique forensic characteristics of each image and serve as feature vectors for detection.

#### 1.2.2. Modeling the Distribution with Gaussian Mixture Model

We model the distribution of forensic self-description embeddings from real images using a Gaussian Mixture Model (GMM). The GMM is a probabilistic model that assumes the data is generated from a mixture of Gaussian distributions with unknown parameters. Formally, the probability density function of the GMM with \( M \) components is:

\[
p(\mathbf{f} \mid \Theta) = \sum_{m=1}^M \pi_m \, \mathcal{N}(\mathbf{f} \mid \boldsymbol{\mu}_m, \boldsymbol{\Sigma}_m),
\]

where:

- \( \Theta = \{ \pi_m, \boldsymbol{\mu}_m, \boldsymbol{\Sigma}_m \}_{m=1}^M \) are the parameters of the GMM.
  - \( \pi_m \) is the mixing coefficient for component \( m \), satisfying \( \sum_{m=1}^M \pi_m = 1 \) and \( \pi_m \geq 0 \).
  - \( \boldsymbol{\mu}_m \) is the mean vector of the \( m \)-th Gaussian component.
  - \( \boldsymbol{\Sigma}_m \) is the covariance matrix of the \( m \)-th Gaussian component.
- \( \mathcal{N}(\mathbf{f} \mid \boldsymbol{\mu}_m, \boldsymbol{\Sigma}_m) \) denotes the multivariate normal distribution.

**Training Phase**:

1. **Dataset Preparation**: Collect a training set \( \mathcal{F}_{\text{real}} = \{ \mathbf{f}_i \}_{i=1}^N \) consisting of forensic self-description embeddings from real images.

2. **Parameter Estimation**: Fit the GMM to \( \mathcal{F}_{\text{real}} \) by maximizing the likelihood function:

   \[
   \Theta^* = \arg\max_{\Theta} \prod_{i=1}^N p(\mathbf{f}_i \mid \Theta).
   \]

   This is typically performed using the Expectation-Maximization (EM) algorithm.

#### 1.2.3. Out-of-Distribution Detection

**Inference Phase**:

For a test image \( I_{\text{test}} \) with embedding \( \mathbf{f}_{\text{test}} \), we compute the likelihood of the embedding under the trained GMM:

\[
p(\mathbf{f}_{\text{test}} \mid \Theta^*) = \sum_{m=1}^M \pi_m^* \, \mathcal{N}(\mathbf{f}_{\text{test}} \mid \boldsymbol{\mu}_m^*, \boldsymbol{\Sigma}_m^*).
\]

**Decision Rule**:

We classify the test image as real or synthetic based on whether \( \mathbf{f}_{\text{test}} \) is likely under the GMM:

- **Real Image**: If \( p(\mathbf{f}_{\text{test}} \mid \Theta^*) \geq \tau \).
- **Synthetic Image**: If \( p(\mathbf{f}_{\text{test}} \mid \Theta^*) < \tau \).

Here, \( \tau \) is a threshold that can be determined using a validation set or set based on desired false positive and false negative rates.

#### 1.2.4. Threshold Selection

Selecting an appropriate threshold \( \tau \) is crucial for balancing detection performance. One approach is to use the quantiles of the likelihoods computed on a validation set of real images. For instance, setting \( \tau \) to the 5th percentile of the validation likelihoods ensures that 95% of real images are correctly classified, allowing for controlled false positive rates.

### 1.3. Advantages of the Proposed Detection Method

- **Zero-Shot Capability**: The method does not require any synthetic images during training, enabling detection of images from unseen AI generators.

- **Robustness to Generative Model Variations**: By modeling the distribution of real images only, the method is inherently robust to the diversity and evolution of generative algorithms.

- **Scalability**: Training the GMM on embeddings is computationally efficient, and the inference process is fast, making it suitable for large-scale applications.

### 1.4. Experimental Validation

We validate the effectiveness of our zero-shot detection method through extensive experiments:

- **Datasets**: Real images from diverse sources and synthetic images generated by various state-of-the-art models (e.g., GANs, diffusion models).

- **Metrics**: Evaluate detection accuracy, precision, recall, and area under the ROC curve (AUC).

- **Results**: Demonstrate high detection rates for synthetic images from both known and previously unseen generators, confirming the discriminative power of the forensic self-description embeddings.

### 1.5. Discussion

The success of our zero-shot detection method underscores the significant differences in forensic microstructures between real and synthetic images. By focusing on the intrinsic properties of real images and modeling their distribution, we effectively identify synthetic images as statistical outliers. This approach aligns with real-world scenarios where new generative models continually emerge, and collecting training data for each is impractical.

### 1.6. Limitations and Future Work

While the proposed method shows strong performance, certain limitations exist:

- **Threshold Sensitivity**: The detection performance depends on the threshold \( \tau \), which may require adjustment for different datasets.

- **Embedding Dimensionality**: High-dimensional embeddings may pose challenges for modeling with GMMs, potentially requiring dimensionality reduction techniques.

Future work may explore adaptive thresholding strategies, alternative probabilistic models for better capturing the embedding distribution, and techniques to enhance the discriminative power of the embeddings.

---

This subsection provides a detailed description of the zero-shot synthetic image detection application, incorporating mathematical rigor as per your instructions. It covers the motivation, methodology, advantages, experimental validation, and discussion of the method. Please let me know if any adjustments are needed or if you would like to proceed to the next application.


# Applications

Leveraging the forensic self-descriptions obtained from individual images, we demonstrate the effectiveness of our method in several applications. In this section, we discuss how these self-descriptions enable:

1. **Zero-Shot Synthetic Image Detection**
2. **Open-Set Synthetic Image Detection and Attribution**
3. **Unsupervised Clustering of Image Sources**

## 1. Zero-Shot Synthetic Image Detection

The significant differences in forensic microstructures between real images (captured by cameras) and synthetic images (generated by AI algorithms) lead to distinctive forensic self-descriptions for each. Building upon this insight, we frame the detection of synthetic images as an **out-of-distribution detection** problem.

### Procedure

After obtaining the forensic self-descriptions as feature vectors (embeddings) for a set of images, we proceed as follows:

1. **Training the Gaussian Mixture Model (GMM):**

   - **Dataset Preparation:** We collect a set of embeddings \( \{ \mathbf{f}_i \} \) extracted from a training set of real images.
   - **Model Training:** We fit a Gaussian Mixture Model \( \mathcal{G} \) to these embeddings to model the distribution of real images in the embedding space.

     Mathematically, the GMM models the probability density function as a weighted sum of Gaussian components:

     \[
     p(\mathbf{f}) = \sum_{c=1}^{C} \pi_c \, \mathcal{N}(\mathbf{f} \mid \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c),
     \]

     where:

     - \( C \) is the number of Gaussian components.
     - \( \pi_c \) are the mixture weights, satisfying \( \sum_{c=1}^{C} \pi_c = 1 \).
     - \( \boldsymbol{\mu}_c \) and \( \boldsymbol{\Sigma}_c \) are the mean and covariance of the \( c \)-th Gaussian component.
     - \( \mathcal{N}(\mathbf{f} \mid \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c) \) is the multivariate normal distribution.

2. **Detection During Inference:**

   - **Embedding Extraction:** For a test image, we extract its forensic self-description embedding \( \mathbf{f}_{\text{test}} \) using the same procedure described earlier.
   - **Probability Estimation:** We compute the likelihood of \( \mathbf{f}_{\text{test}} \) under the GMM:

     \[
     p_{\mathcal{G}}(\mathbf{f}_{\text{test}}) = \sum_{c=1}^{C} \pi_c \, \mathcal{N}(\mathbf{f}_{\text{test}} \mid \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c).
     \]

   - **Classification Decision:**

     - **Thresholding:** We set a threshold \( \tau \) on the likelihood. If \( p_{\mathcal{G}}(\mathbf{f}_{\text{test}}) \geq \tau \), we classify the image as **real**; otherwise, we classify it as **synthetic**.
     - **Out-of-Distribution Detection:** Since the GMM is trained only on real images, embeddings from synthetic images are expected to have low likelihoods under the model, effectively being identified as out-of-distribution samples.

### Rationale

- **Distinct Embedding Distributions:** Real images and synthetic images produce embeddings that occupy different regions in the embedding space due to the inherent differences in their forensic microstructures.
- **Gaussian Mixture Modeling:** By modeling the distribution of real image embeddings, the GMM captures the variability and structure inherent in real forensic self-descriptions.
- **Likelihood Thresholding:** Using a likelihood threshold allows for a probabilistic decision boundary, providing flexibility in controlling the trade-off between false positives and false negatives.

### Practical Considerations

- **Choice of Number of Components \( C \):** The number of Gaussian components can be determined using model selection techniques such as the Bayesian Information Criterion (BIC) or cross-validation.
- **Threshold Selection:** The threshold \( \tau \) can be set based on the desired operating point or determined empirically using a validation set of real images.
- **Feature Normalization:** Prior to training the GMM, embeddings may be normalized (e.g., using z-score normalization) to improve modeling accuracy.

### Advantages of Our Approach

- **Zero-Shot Capability:** The method does not require any synthetic images during training, enabling detection of images from unseen AI generators.
- **Adaptability:** By modeling only the distribution of real images, the approach remains robust as new generative models emerge.
- **Simplicity and Efficiency:** The use of GMMs allows for efficient computation and straightforward implementation.

### Summary

By framing synthetic image detection as an out-of-distribution detection problem and leveraging the distinctive forensic self-descriptions of real images, our method achieves accurate zero-shot detection of AI-generated images. The Gaussian Mixture Model serves as an effective tool to model the distribution of real image embeddings and identify deviations indicative of synthetic origins.
\end{comment}









==> sections/Background_v0.tex <==
\section{Background and Related Work}

\textcolor{red}{\textbf{This is automatically generated by ChatGPT. The content may not be accurate. References may not exist.}}

The rapid advancement of generative models has led to the proliferation of highly realistic synthetic images, posing significant challenges for detection and attribution. In response, researchers have developed various methods to distinguish synthetic images from real ones. This section reviews relevant literature in five key areas: steganalysis and forensic microstructures, supervised detection methods, open-set source attribution, zero-shot detection techniques, and unsupervised clustering approaches.

\subheader{Steganalysis and Forensic Microstructures in Synthetic Image Detection}
Steganalysis is the study of detecting hidden information within digital media. Traditionally focused on uncovering concealed messages in images, steganalysis techniques analyze statistical anomalies and artifacts introduced during data embedding. This field has significantly influenced synthetic image detection by emphasizing the importance of forensic microstructures—subtle patterns or artifacts embedded in images during their creation or manipulation.

In the context of synthetic image detection, forensic microstructures are exploited to differentiate between real and AI-generated images. Early approaches utilized handcrafted features to capture these microstructures. For instance, Fridrich and Kodovský introduced rich models for steganalysis that analyze residuals obtained from high-pass filters to detect hidden information, laying the groundwork for detecting synthetic artifacts. While these methods are capable of capturing subtle artifacts undetectable by the human eye, they often rely on specific assumptions about the types of artifacts present, which may not generalize well across different synthetic content.

With the rise of deep learning, convolutional neural networks (CNNs) have been employed to automatically learn and extract forensic features from images. Bayar and Stamm proposed a CNN architecture designed to suppress image content and emphasize manipulation artifacts, improving detection performance. Although CNN-based methods can effectively detect synthetic images from known generators, their performance can degrade when faced with images from unseen generative models due to overfitting on known artifacts.

\subheader{Supervised Methods for Synthetic Image Detection}
Supervised learning approaches train models using labeled datasets comprising real images and synthetic images generated by specific AI models. The objective is to learn discriminative features that can distinguish between real and synthetic images based on patterns learned during training. Yu et al. trained CNNs to detect GAN-generated faces by learning differences in color patterns and texture inconsistencies, while Marra et al. focused on detecting DeepFake videos by analyzing compression artifacts introduced during the generation process.

These supervised methods often achieve high accuracy on test data similar to the training set, leveraging powerful deep learning models for feature extraction. However, they struggle to generalize to images from unseen generators. The models tend to overfit to the artifacts present in the training data, and when presented with synthetic images from new generators, their detection capabilities diminish significantly. This limitation makes them ineffective in open-set scenarios where new types of synthetic images continually emerge. Additionally, supervised methods require extensive labeled data for each type of synthetic generator, which is impractical given the rapid development of new generative models.

\subheader{Open-Set Synthetic Image Source Attribution Methods}
To overcome the limitations of supervised methods, researchers have explored open-set recognition techniques for synthetic image detection and source attribution. Open-set methods aim to correctly classify samples from known classes while effectively identifying samples from unknown classes as novel. Bendale and Boult's OpenMax is a notable approach that extends traditional softmax classifiers by incorporating a model of activations for known classes to estimate the probability of an input belonging to an unknown class.

In synthetic image detection, open-set methods provide a mechanism for both detection and source attribution of known generators while flagging images from unseen generators as unknown. They are better at handling images from unknown sources compared to purely supervised methods. However, their detection performance depends heavily on the feature representations learned from known classes. If the features do not generalize well to unknown synthetic images, the methods may fail to detect them effectively. Additionally, open-set methods require careful calibration to balance false positives and false negatives, which can be challenging in practice.

\subheader{Zero-Shot Synthetic Image Detection Methods}
Zero-shot detection methods aim to identify synthetic images without prior exposure to specific generative models during training. These methods seek to learn generalizable features that can differentiate real images from any synthetic images based on inherent differences in their data distributions. Wang et al. proposed leveraging inconsistencies in frequency domain representations by analyzing disparities in spectral distributions between real and synthetic images. Another approach by Gragnaniello et al. utilized pre-trained models on natural image datasets to extract embeddings and applied anomaly detection techniques to identify synthetic images.

Zero-shot methods do not require labeled synthetic images from every possible generator, making them more adaptable to new and unseen generators. However, there is no guarantee that the learned features will capture all relevant discrepancies between real and synthetic images. The performance of zero-shot methods can vary significantly depending on the characteristics of new generative models. They may miss subtle artifacts introduced by advanced generators, especially if those artifacts do not align with the features the model has learned to detect.

\subheader{Unsupervised Clustering of Real and Synthetic Sources}
Unsupervised clustering approaches attempt to group images based on intrinsic similarities without relying on labeled data. In synthetic image detection, the goal is to cluster real images separately from synthetic ones and potentially further cluster synthetic images by their source generators. To the best of our knowledge, there are limited studies that focus on unsupervised clustering for synthetic image detection. This is because the performance of unsupervised clustering methods heavily relies on the quality of the learned representations and the ability to distinguish subtle differences between real and synthetic images. Without explicit supervision, these methods may struggle to capture the forensic microstructures that differentiate synthetic images from real ones.

In summary, although significant progress has been made in detecting synthetic images, existing methods often face challenges in generalizing to new, unseen generative models. Supervised methods are limited by their dependence on labeled data from known generators and struggle with overfitting. Open-set and zero-shot approaches attempt to address these limitations but may not fully capture the nuances introduced by novel generators, as their performance depends on the generalizability of the learned features. Unsupervised clustering remains difficult due to its reliance on high-quality embeddings that can distinguish between classes without prior knowledge.

Our work addresses these limitations by proposing a method that constructs a self-contained, compact model of the underlying forensic microstructures for each image. By focusing on the intrinsic forensic properties unique to each image, our approach enables accurate zero-shot detection, open-set source attribution, and unsupervised clustering without prior exposure to specific synthetic generators. This method leverages the differences in forensic microstructures between real and synthetic images, providing a robust solution to the challenges faced by existing detection techniques.


==> sections/Background_v1.tex <==
\section{Background and Related Work}

The proliferation of highly realistic synthetic images generated by advanced AI models has posed significant challenges for detection and attribution. Researchers have explored various methods to distinguish synthetic images from real ones, drawing from steganalysis, supervised learning, open-set recognition, zero-shot detection, and unsupervised clustering. This section provides a concise overview of these approaches, highlighting their methodologies, strengths, and limitations.

\subheader{Steganalysis and Forensic Microstructures in Synthetic Image Detection}
Steganalysis, the study of detecting hidden information within digital media, has significantly influenced synthetic image detection by emphasizing the importance of forensic microstructures—subtle patterns embedded in images during creation or manipulation. Early methods utilized handcrafted features, such as high-pass filters and statistical models, to capture these microstructures. With the advent of deep learning, convolutional neural networks (CNNs) have been employed to automatically learn and extract forensic features that can be used for a variety of forensic tasks. In the context of synthetic image detection, forensic microstructures are often extracted and modelled using a deep neural network to differentiate between real and AI-generated images.

\subheader{Supervised Methods for Synthetic Image Detection}
Supervised learning approaches train models using labeled datasets comprising real images and synthetic images generated by specific AI models. The objective is to learn discriminative features that can distinguish between real and synthetic images based on patterns learned during training. For instance, Yu et al. trained CNNs to detect GAN-generated faces by learning differences in color patterns and texture inconsistencies. These supervised methods often achieve high accuracy on test data similar to the training set, but struggle to generalize to images from unseen generators. This is because different generative models introduce unique artifacts that may not be captured by the learned features. This limitation makes them ineffective in open-set scenarios where new types of synthetic images continually emerge.

\subheader{Open-Set Synthetic Image Source Attribution}
To address the limitations of supervised methods, researchers have explored open-set recognition techniques that aim to detect and attribution the source of known generators while flagging images from unseen generators as unknown. They are better at handling images from unknown sources compared to purely supervised methods. However, their detection performance depends heavily on the feature representations learned from known classes. If the features do not generalize well to unknown synthetic images, the methods may fail to detect them effectively. Additionally, open-set methods require careful calibration to balance false positives and false negatives, which can be challenging in practice.

\subheader{Zero-Shot Synthetic Image Detection}
Zero-shot detection methods aim to identify synthetic images without prior exposure to specific generative models during training by learning generalizable features that differentiate real images from synthetic ones based on inherent data distribution differences. Techniques include analyzing inconsistencies in frequency domain representations or leveraging embeddings from pre-trained models on natural images. While zero-shot methods do not require labeled synthetic images from every generator and are more adaptable to new and unseen models, their performance can vary significantly. There is no guarantee that the learned features will capture all relevant discrepancies, and as generative techniques improve over time, they may produce artifacts that these methods fail to detect.

\subheader{Unsupervised Clustering of Real and Synthetic Sources}
Unsupervised clustering approaches attempt to group images based on intrinsic similarities without relying on labeled data. In synthetic image detection, the goal is to cluster real images separately from synthetic ones and potentially further cluster synthetic images by their source generators. To the best of our knowledge, there are limited studies that focus on unsupervised clustering for synthetic image detection. This is because the performance of unsupervised clustering methods heavily relies on the quality of the learned representations and the ability to distinguish subtle differences between real and synthetic images. Without explicit supervision, these methods may struggle to capture the forensic microstructures that differentiate synthetic images from real ones.

In summary, while significant progress has been made in detecting synthetic images, existing methods often face challenges in generalizing to new, unseen generative models. Supervised methods are limited by their dependence on labeled data from known generators and struggle with overfitting. Open-set and zero-shot approaches attempt to address these limitations but may not fully capture the nuances introduced by novel generators due to their reliance on the generalizability of learned features. Unsupervised clustering remains challenging because of its dependence on high-quality embeddings that can distinguish between classes without prior knowledge. Our work addresses these limitations by constructing a self-contained, compact model of the underlying forensic microstructures for each image, enabling accurate zero-shot detection, open-set source attribution, and unsupervised clustering without prior exposure to specific synthetic generators.




==> sections/ExperimentalSetup_v0.tex <==
\section{Experimental Setup}

To demonstrate the utility of our proposed forensic self-descriptions on each of the three applications: (1) zero-shot detection of synthetic images, (2) open-set source attribution of synthetic images, and (3) unsupervised clustering of image sources, we conducted three sets of experiments. We describe the datasets, evaluation metrics, and implementation details for each of these experiments below.

\subsection{Datasets}

In order to conduct our experiments, we pooled together a large composite dataset of real and synthetic images from various publicly available sources and our own sources. The real images are pooled from four publicly available datasets: (1) COCO2017~\citethis, (2) ImageNet-1k~\citethis, (3), ImageNet-22k~\citethis, and (4) MISL Image Database (MIDB)~\citethis. The synthetic images are collected from three different public datasets: (1) Open-set Synthetic Image Attribution (OSIA) dataset~\citethis, (2) Diffusion Model Image Detection (DMID) dataset~\citethis, and (3) Synthbuster dataset~\citethis. In aggregate, our set of synthetic images includes 24 different generators, covering a wide range of open-source, closed-source and proprietary generative techniques, such as:
ProGAN~\citethis,
Projected GAN~\citethis,
StyleGAN [1, 2, 3]~\citethis,
BigGAN~\citethis,
GigaGAN~\citethis,
EG3D~\citethis,
Taming Transformers (Tam.Xf)~\citethis,
GLIDE~\citethis,
Guided Diffusion (GD)~\citethis,
Latent Diffusion (LD)~\citethis,
Stable Diffusion (SD) [1.3, 1.4, 1.5, 2.1, XL, 3.0]~\citethis,
DALLE [M, 2, 3]~\citethis,
Midjourney (MJ) [v5, v6]~\citethis,
Adobe Firefly~\citethis
.
%
More details on the exact composition of these datasets and the number of images per generator are provided in the supplementary material.

\subsection{Setup for Zero-Shot Detection Experiment}

To evaluate the performance of ours and competing methods in detecting synthetic images in a zero-shot setting, we split our composite dataset into a training set and a test set. The training set consists of real images only, while the test set contains both real and synthetic images. After training our model on the training set, we evaluated its performance on the test set.

Following methodologies from prior works~\citethis, we computed performance metrics for each individual pair of real vs. a synthetic generator. In total, we have $4 \times 24 = 96$ dataset pairs. As space is limited, we provide the average performance metrics across all pairs with respect to a real source in the main text and full results for each pair in the supplementary material.

\subheader{Evaluation Metrics}
To enable direct comparison with prior works~\citethis, we compute the Area Under the ROC curve (AUC) to fairly compare methods irrespective of detection thresholds.

\subheader{Competing Methods}
We compare our method against eight state-of-the-art methods for synthetic image detection, ranging from traditional classifier approaches like CNNDet~\citethis \& PatchForensics~\citethis, gradient-based methods like LGrad~\citethis, embedding-distance-based methods like UFD~\citethis, training-free methods like DE-FAKE~\citethis, and reconstruction-error-based methods like Aeroblade~\citethis \& ZED~\citethis.


\subsection{Setup for Open-Set Attribution Experiment}

To test the ability of our method and others to attribute synthetic images to their respective sources in an open-set setting, we followed a procedure established by other open-set work~\citethis. First, we selected a subset of 9 sources (1 real + 8 synthetic sources) from our pooled dataset and split them into 5 known (Imagenet-1k, StyleGAN, StyleGAN3, SD 1.4, ProGAN) and 4 unknown sources (StyleGAN2, SD 3, DALLE 3, Firefly). For each known source, we further split the images into a training set and a test set. Our method and competing methods are trained on the same training set and evaluated on the test set which includes images from both known and unknown sources.

\subheader{Evaluation Metrics}
Following other open-set works~\citethis, we show (1) how accurate the methods are in at attributing images from known sources by computing the average accuracy across all known sources, and (2) how well the methods can determine if an image is from a known or unknown source by computing the Area Under the Correct Rejection Rate curve (AU-CRR)~\citethis. We additionally report the Area Under the Open Set Classification Rate curve (AU-OSCR)~\citethis which summarizes the performance of two aspects of an open-set method.


\subheader{Competing Methods}
We compare our method against three state-of-the-art methods specifically designed for open-set synthetic image source attribution: Barni~\citethis, Fang~\citethis, POSE~\citethis, two metric-learning-based methods designed for image forensic tasks: FSM~\citethis, EXIFNet~\citethis, and two methods which produce a generic embedding for vision tasks: CLIP~\citethis, ResNet-50~\citethis trained on ImageNet-1k. For methods which only produces a generic embedding, we apply the same open-set procedure proposed in Sec.~\ref{sec:application_openset} to their produced embeddings and evaluate their performance.


\subsection{Setup for Clustering Experiment}

To evaluate the performance of our method and competing methods in clustering images based on their source, we selected a subset of 8 sources from our composite dataset (Real: Imagenet-1k; Synthetic: ProGAN, StyleGAN3, GLIDE, SD 1.5, DALLE 3, MJ v6, and Firefly). We intentionally chose sources that represent distinct generative technologies because we wanted to see how reliable our method is in its ability to identify a new source. Since our method is applied in an unsupervised manner, we do not require any training data. We directly apply our method to the images from the selected sources and evaluate the clustering performance.


\subheader{Evaluation Metrics}
Conforming to other clustering works~\citethis, we show (1) how accurate the clustering is by computing the average accuracy across all sources, (2) how pure the clusters are by computing the Average Purity score, and (3) how well the clusters align with the ground truth irrespective of the number of clusters by computing the Normalized Mutual Information (NMI) score. Additionally, we present these three metrics over different integer multiples of the true number of sources to show the robustness of the methods.

\subheader{Competing Methods}
Since there are no existing methods specifically designed for unsupervised clustering of synthetic images, we compare our method's performance against the top-4 performing methods in the zero-shot detection experiment: NPR~\citethis, UFD~\citethis, DE-FAKE~\citethis \& CnnDet~\citethis, as well as 3 metric-learning-based methods: FSM~\citethis, EXIFNet~\citethis \& Barni et. al~\citethis, and 2 methods which produce a generic embedding for vision tasks: CLIP~\citethis, ResNet-50~\citethis (trained on ImageNet-1k). To perform clustering with these methods, we first extract the embeddings produced from their models, either by using a specified embedder network, or by using the penultimate layer before the classification layer of the model. We then apply K-means clustering using either the specified metric network if provided, or the Euclidean distance metric. This ensures a fair comparison across all methods.









==> sections/ExperimentalSetup_v1.tex <==
\section{Experimental Setup}

We evaluated the effectiveness of our forensic self-description across three tasks: (1) zero-shot synthetic image detection, (2) open-set synthetic image attribution, and (3) unsupervised clustering of image sources. Below, we describe the datasets, metrics, and experimental setups.



\subsection{Datasets}
\label{sec:datasets}
To conduct our experiments, we pooled together a large composite dataset of real and synthetic images from various publicly available sources. Real images are drawn from: (1) COCO2017~\cite{coco}, (2) ImageNet-1k~\cite{imagenet}, (3), ImageNet-22k~\citethis, and (4) MISL Image Database (MIDB)~\citethis. Synthetic images come from: (1) the OSSIA dataset ~\citethis, (2) the DMID dataset~\citethis, and (3) Synthbuster dataset~\cite{Synthbuster}. In aggregate, our set of synthetic images includes 24 generators across diverse architectures. Some notable ones are:
ProGAN~\cite{progan},
StyleGAN [v1 to 3]~\cite{stylegan,stylegan2,stylegan3},
GigaGAN~\cite{Gigagan},
EG3D~\cite{eg3d},
GLIDE~\cite{glide},
Stable Diffusion (SD) [v1.3 to 3.0]~\cite{stablediff},
DALLE [M, 2, 3]~\cite{dallemini,dalle2,dalle3},
Midjourney (MJ) [v5, v6]~\cite{Midjourney},
Adobe Firefly~\cite{AdobeFirefly}
.
%
Full details on dataset composition are available in the supplementary material.


\subsection{Setup for Zero-Shot Detection Experiment}

To assess zero-shot detection, we divided the composite dataset into a training set of real images and a test set of both real and synthetic images. We measured performance across 96 real-synthetic dataset pairs. As space is limited, we provide the average performance metrics across all pairs with respect to a real source in the main text and full results for each pair in the supplementary material.

\subheader{Evaluation Metrics}
We report the average AUC (Area Under the ROC curve) for direct comparison with prior works.


\subheader{Competing Methods}
%We compare our method against eight state-of-the-art approaches, ranging from binary classifier approaches like CNNDet~\citethis \& PatchForensics~\citethis, gradient-based methods like LGrad~\citethis, embedding-distance-based methods like UFD~\citethis, training-free methods like DE-FAKE~\citethis, and reconstruction-error-based methods like Aeroblade~\citethis \& ZED~\citethis.
We compared our method to eight state-of-the-art approaches, including CNNDet~\cite{CNNDet}, PatchForensics~\cite{PatchFor}, LGrad~\cite{LGrad}, UFD~\cite{UFD}, DE-FAKE~\cite{DE-Fake}, Aeroblade~\cite{Aeroblade}, and ZED~\cite{Zed}.




\subsection{Setup for Open-Set Attribution Experiment}

For open-set source attribution, we selected 9 sources (1 real and 8 synthetic), dividing them into 5 known (Imagenet-1k, StyleGAN, StyleGAN3, SD 1.4, ProGAN) and 4 unknown sources (StyleGAN2, SD 3, DALLE 3, Firefly). Models were trained on known sources and tested on both known and unknown sources.

\subheader{Evaluation Metrics}
Following other open-set works~\cite{POSE, OSCR, Fang_2023_BMVC}, we show (1) the average accuracy across all known sources, and (2) the Area Under the Correct Rejection Rate curve (AU-CRR)~\cite{POSE, Fang_2023_BMVC}, and (3) the Area Under the Open Set Classification Rate curve (AU-OSCR)~\cite{POSE, OSCR}.


\subheader{Competing Methods}
We compare our method against three state-of-the-art methods designed for this task: Abady et. al~\cite{Abady}, Fang et. al~\cite{Fang_2023_BMVC}, POSE~\cite{POSE}, two metric-learning-based methods designed for image forensic: FSM~\cite{FSM}, EXIFNet~\cite{ExifNet}, and two methods which produce embeddings for computer vision: CLIP~\cite{CLIP}, and a ResNet-50~\cite{resnet} trained on ImageNet1k. For methods which only produces a generic embedding, we apply the same open-set procedure proposed in Sec.~\ref{sec:application_openset} to their produced embeddings.


\subsection{Setup for Clustering Experiment}

To evaluate clustering, we used 8 sources representing distinct generation techniques (Real: ImageNet-1k; Synthetic: ProGAN, StyleGAN3, GLIDE, SD 1.5, DALLE 3, MJ v6, Firefly). Our method, applied in an unsupervised manner, does not require training data.


\subheader{Evaluation Metrics}
Conforming to other clustering works~\citethis, We present clustering accuracy, purity, and NMI (Normalized Mutual Information), measured across different integer multiples of the true number of sources to show the robustness of the methods.

\subheader{Competing Methods}
We evaluated our method against the top four zero-shot methods: NPR~\cite{NPR}, UFD~\cite{UFD}, DE-FAKE~\cite{DE-Fake} \& CnnDet~\cite{CNNDet}, 3 metric-learning-based methods: FSM~\cite{FSM}, EXIFNet~\cite{ExifNet} \& Abady et. al~\cite{Abady}, as well as general vision embeddings: CLIP~\cite{CLIP}, and ResNet-50~\cite{resnet} trained on ImageNet1k. For each method, we extracted embeddings from either the specified embedder network or the penultimate layer and applied K-means clustering using Euclidean distance or the method’s provided metric.









==> sections/ExtractForensicResiduals_v0.tex <==
\subsection{Forensic Microstructures as Residuals}

To obtain the forensic self-description for each image, we first need to extract the forensic microstructures present within it. We achieve this by proposing a simple additive model where the pixel values in an image are considered as the sum of the scene content, the forensic microstructures, and uncorrelated noise. Mathematically, this model is expressed as:
\begin{equation}
    I(x,y) = S(x,y) + \Psi(x,y) + \epsilon(x,y),
\end{equation}
where $I(x,y)$ is the observed pixel value at location $(x,y)$ in image $I$, $S(x,y)$ represents the scene content at location $(x,y)$, $\Psi(x,y)$ denotes the forensic microstructures introduced during the image formation and processing pipeline, $\epsilon(x,y)$ is some amount of uncorrelated Gaussian white noise.

Our goal is to isolate the forensic microstructures $\Psi(x,y)$ from the observed image $I(x,y)$. Since $\Psi(x,y)$ is not directly observable, we need to approximate $S(x,y)$. Inspired by prior work, we achieve this by modeling $S(x,y)$ using a parametric function $F$ with parameters $\mathbf{W}_{\theta}$:
\begin{equation}
    \hat{S}(x,y) = F(I, \mathbf{W}_{\theta})(x,y).
\end{equation}
By substituting $\hat{S}(x,y)$ into our additive model, we obtain a residual after subtracting the estimated scene content from the observed image. This residual approximate the forensic microstructures present in the image:
\begin{equation}
    \hat{\Psi}(x,y) = I(x,y) - \hat{S}(x,y).
\end{equation}
In practice, the forensic microstructures are akin to a multiplexed signal composed of intertwined patterns within an image. To recover and analyze these individual patterns, we demultiplex the signal using multiple filters, each designed to extract a specific aspect of the microstructures. This decomposition captures all facets of the forensic characteristics, providing a comprehensive representation essential for accurate detection and attribution.

\begin{comment}
    In practice, the forensic microstructures in images can be likened to a multiplexed signal, where multiple underlying patterns are combined into a single composite signal during the image formation process. To effectively analyze and recover these distinct components, we need to demultiplex the signal using multiple filters, each tailored to isolate a specific aspect of the microstructures. By applying a diverse set of filters, we decompose the complex forensic signal into its constituent parts, allowing us to capture all facets of the microstructures present in the image. This approach ensures a comprehensive representation of the forensic characteristics, which is essential for accurate detection and attribution tasks.
\end{comment}


\subheader{Modeling Scene Content}

Here we propose $F$ using a set of linear predictive filters $\{\mathbf{W}_\theta^k\}_{k=1}^K$ that predict the value of a center pixel based on its surrounding neighborhood. These filters leverage the spatial correlations inherent in natural images to estimate the scene content at each pixel location. The prediction for the $k$-th filter is given by:
\begin{equation}
    \hat{S}^k(x,y) = \sum_{(i,j) \in \mathcal{M}} \mathbf{W}_\theta^k(i,j) \cdot I(x + i, y + j),
\end{equation}
where $\mathcal{M}$ is the set of offsets corresponding to the neighborhood pixels around $(x,y)$ excluding the $(x,y)$ pixel itself, $\mathbf{W}_\theta^k(i,j)$ are the weights of the $k$-th filter for offset $(i,j)$, and $S^k(x,y)$ is the prediction of the pixel value at $(x,y)$ using the $k$-th filter. In practice, inspired by the work of Bayar and Stamm\citethis, we utitlize a special convolutional layer that is constrained such that the center kernel weight is set to $0$ and the sum of the kernel weights is $1$ to preserve the energy of the input image.

Then, the residual for each filter are computed as:
\begin{equation}
    \hat{\Psi}^k(x,y) = I(x,y) - \hat{S}^k(x,y)
\end{equation}
Each residual $\hat{\Psi}^k(x,y)$ captures a different aspect of the forensic microstructures. Together, the set of residuals $\{\hat{\Psi}^k(x,y)\}_{k=1}^K$ represents the comprehensive forensic microstructures present in the image.

\subheader{Optimization Objective for Learning $\mathbf{W}_\theta$}

In order to both effectively separate the scene content from the input image and ensure that the resulting residuals capture all essential aspects of the image's forensic microstructures, our optimization objective must contain two key components. First, we need to minimize the residuals across all filters to ensure that the scene content is accurately predicted. This results in the following loss term $\mathcal{L}_F$:
\begin{equation}
    \mathcal{L}_F(\mathbf{W}_\theta) = \sum_{k=1}^K \sum_{x,y} \left( \hat{\Psi}^k(x,y) \right)^2.
\end{equation}
This term encourages the filters to accurately predict the scene content, thereby minimizing the residuals, which predominantly capture the forensic microstructures and noise.

Second, we need to ensure that the filters are diverse and do not become redundant. To this end, we introduce a spectral diversity regularization term that encourages the filters to be as linearly independent as possible, maximizing the diversity of information captured.

To do this, we first construct a filter matrix $\mathbf{W} \in \mathbb{R}^{K \times N}$ by reorienting the weights of each filter into a vector:
\begin{equation}
    \mathbf{W} =
    \begin{bmatrix}
        \mathrm{vec}(\mathbf{W}_\theta^1)^\top \\
        \mathrm{vec}(\mathbf{W}_\theta^2)^\top \\
        \vdots \\
        \mathrm{vec}(\mathbf{W}_\theta^K)^\top
    \end{bmatrix},
\end{equation}
in which $N = |\mathcal{M}| >> K$ is the number of elements in each filter (the size of the neighborhood). We then perform the Singular Value Decomposition (SVD) on $\mathbf{W}$ to obtain the set of singular values $\left\{ \sigma_i \right\}_{i=1}^K$. Finally, the spectral diversity regularization term is defined as:
\begin{equation}
    \mathcal{L}_{\text{diversity}}(\mathbf{W}_\theta) = - \sum_{i=1}^{K} \log(\sigma_i + \epsilon),
\end{equation}
where $\epsilon$ is a small constant to prevent numerical instability. This regularization term penalizes filter configurations where singular values are small, which would indicate that some filters are linearly dependent on others. By minimizing $\mathcal{L}_{\text{diversity}}$, we encourage the filters to be as diverse as possible.

By combinining the two terms, we obtain the overall optimization objective for learning the predictive filters:
\begin{equation}
    \mathbf{W}_\theta^* = \arg\min_{\mathbf{W}_\theta} \left[ \mathcal{L}_F(\mathbf{W}_\theta) + \lambda \mathcal{L}_{\text{diversity}}(\mathbf{W}_\theta) \right],
\end{equation}
where $\lambda$ is a hyperparameter that balances the two terms. By solving this optimization problem over a diverse set of real images, we obtain a set of predictive filters $\mathbf{W}_\theta^*$ that effectively approximate the scene content and isolate the forensic microstructures from any given image. 


% \textit{(Likely omit) These extracted forensic microstructures serve as the foundation for constructing the forensic self-description of each image, which we will discuss in the following subsection.}

















































==> sections/ExtractForensicResiduals_v1.tex <==
\subsection{Forensic Microstructures Extraction}
\label{sec:method_forensic_residuals}

% 1. Significant prior research has shown that the processes at which an image is formed leave behind forensic microstructures that can be used to identify the source of the image.
% 2. Hence, to perform various forensic tasks, it is essential to produce an accurate description of these forensic microstructures.
% 3. However, these microstructures are inherently unobservable, making it challenging to directly model them.
% 4. To overcome this problem, we propose a simple additive model of an image, in which an image's resulting pixel values are the sum of three independent components: the scene content, the forensic microstructures, and image formation noise.
% 5. Using this model, we can isolate the forensic microstructures by approximating the scene content and subtracting it from the observed image.
% 6. This subtraction results in a residual that captures the forensic microstructures present in the image and some estimation noise + image formation noise.
% 7. In practice, however, it is very challenging to perfectly approximate the scene content due to the infinite number of possible configurations of pixel values in an image. Therefore, the residual may not fully capture the forensic microstructures, making it difficult to accurately describe them.
% 8. To address this challenge, instead of using a single model to predict the scene content, we propose using a set of diverse models, each capturing a different aspect of the scene content. This ensemble of models allow us to extract not just one residual, but multiple reisiduals, each capturing a different characteristic of the forensic microstructures.
% 9. This is akin to reconstructing a 3D object (forensic microstructures) from 2D images (residuals) taken from different angles. By combining the information from multiple, equally spaced angles, we can obtain a more accurate representation of the 3D object.
% 10. In our instance, inspired by prior work in forensics, we approximate the scene content using a series of linear predictive filters that predict the value of a center pixel based on its surrounding neighborhood.

Prior research has shown that the processes at which an image is formed leave behind unique forensic microstructures that can be used to identify its source. Hence, to detect and attribute the source of synthetic images, it is essential to produce an accurate description of these forensic microstructures. However, since they are inherently unobservable,  it's challenging to directly analyze them.

To overcome this problem, we propose a simple additive model of an image, in which an image's observed pixel values $I$ are the sum of: the scene content $S$, the forensic microstructures $\Psi$, and some image formation noise $\epsilon$. Mathematically, this model is expressed as:
\begin{equation}
    I(x,y) = S(x,y) + \Psi(x,y) + \epsilon(x,y),
\end{equation}
where $(x, y)$ are the 2D pixel coordinates.

Using this model, we can isolate the forensic microstructures by approximating the scene content and subtracting it from the observed image. This subtraction results in a residual that captures the forensic microstructures present in the image, along with estimation and image formation noise:
\begin{align}
    \label{eq:residual}
    r(x, y) &= I(x, y) - \hat{S}(x, y) \\
            &= \Psi(x,y) + \epsilon(x,y) + \epsilon_\Psi(x,y),
\end{align}
where $r(x, y)$ is the residual that contains forensic microstructures, and $\epsilon_\Psi(x, y)$ is the estimation noise.

In practice, however, it is challenging to perfectly approximate the scene content due to the infinite number of possible configurations of pixel values in an image. Therefore, the residual may not fully capture the underlying forensic microstructures.

To address this challenge, instead of using a single model to predict the scene content, we propose using a diverse set of models. These models then extract a diverse set of residuals, each capturing a different characteristic of the forensic microstructures. This is akin to reconstructing a 3D object from 2D images taken from different angles. By combining the information captured by multiple images at diverse angles, we can more accurately reconstruct the 3D object. Mathematically, this is expressed as:
\begin{equation}
    r_k(x,y) = I(x,y) - \hat{S}_k(x,y), \quad k = 1, 2, \ldots, K,
\end{equation}

In this paper, inspired by prior work, we approximate the scene content using a series of $K$ learnable linear predictive filters $\mathbf{W} = \{\mathbf{W}_k\}_{k=1}^K$ that predict the value of a center pixel based on its surrounding neighborhood, such that:
\begin{equation}
    \hat{S}_k(x,y) = \sum_{(i,j) \in \mathcal{M}} \mathbf{W}_k(i,j) \cdot I(x + i, y + j),
\end{equation}
where $\mathcal{M}$ is the set of offsets in the $M \times M$ neighborhood pixels around $(x,y)$ excluding $(0, 0)$. We implement these filters by constraining a convolutional layer such that the center kernel weight is always set to $0$ and the sum of all kernel weights is $1$ to preserve the energy of the input image.

To learn $\mathbf{W}$, we first need to train it to minimize the total energy across all residuals. This results in the following loss term $\mathcal{L}_E$:
\begin{equation}
    \mathcal{L}_E(\mathbf{W}) = \sum_{k=1}^K \sum_{x,y} \left( I(x,y) - \hat{S}_k(x,y) \right)^2.
\end{equation}
However, this loss term alone may produce filters that are redundant. To prevent this, we introduce a novel spectral diversity regularization term that encourages the filters to be as linearly independent as possible, maximizing the diversity of information captured. Returning to our earlier analogy, this is akin to making sure that the captured 2D images are equally spaced around the 3D object.

To do this, we first construct a matrix $\mathbf{D} \in \mathbb{R}^{K \times (M^2)}$ by reorienting the weights of each filter into a vector:
\begin{equation}
    \mathbf{D} =
    \begin{bmatrix}
        \mathrm{vec}(\mathbf{W}_1)^\top \\
        \mathrm{vec}(\mathbf{W}_2)^\top \\
        \vdots \\
        \mathrm{vec}(\mathbf{W}_K)^\top
    \end{bmatrix},
\end{equation}
in which $M^2 >> K$. We then perform the Singular Value Decomposition (SVD) on $\mathbf{D}$ to obtain the set of singular values $\left\{ \sigma_i \right\}_{i=1}^K$. Finally, the spectral diversity regularization term is defined as:
\begin{equation}
    \mathcal{L}_{\text{diversity}}(\mathbf{D}) = - \sum_{i=1}^{K} \log(\sigma_i + \alpha),
\end{equation}
where $\alpha$ is a small constant to prevent numerical instability. This term penalizes filter configurations where singular values are small, which would indicate that some filters are linearly dependent on others. By minimizing $\mathcal{L}_{\text{diversity}}$, we encourage the filters to be as diverse as possible.

By combinining the two terms, we obtain the overall optimization objective for learning the predictive filters:
\begin{equation}
    \mathbf{W}^* = \arg\min_{\mathbf{W}} \left[ \mathcal{L}_E(\mathbf{W}) + \lambda \mathcal{L}_{\text{diversity}}(\mathbf{W}) \right],
\end{equation}
where $\lambda$ is a hyperparameter that balances the two terms. By solving this optimization problem over a diverse set of real images, we obtain a set of predictive filters $\mathbf{W}^*$ that approximates the scene content and effectively isolates the forensic microstructures plus noise from any given image.




==> sections/Implementation_v0.tex <==






==> sections/Intro_v0.tex <==
\section{Introduction}
\label{sec:intro}

The rapid proliferation of AI-generated media has emerged as a significant challenge for society, with new synthetic image generators being introduced at an accelerating pace. These advances have enabled the creation of hyper-realistic visual content, raising concerns about misinformation, security, and authenticity. Recent developments in deep learning-based generative models such as StyleGAN and Stable Diffusion have only intensified these challenges, necessitating robust forensic techniques for differentiating between real and AI-generated images.

Prior research has made substantial progress in supervised classification of synthetic media, achieving strong performance in distinguishing real images from those generated by models seen during training. However, this performance often falters when classifiers encounter images from previously unseen generators, particularly when these generators belong to fundamentally different architectural families. For instance, models trained to recognize artifacts in images produced by StyleGAN may struggle to detect those generated by Stable Diffusion, as each architecture leaves behind distinct forensic traces. Since existing methods do not have access to future generators during training, they naturally learn to focus on discriminative features present in the current training dataset. This process leads them to overlook non-discriminative features that could become important for identifying images from future, unseen generators. As a result, these models often lack the generalizability needed to be effective in real-world, open-set scenarios, where the diversity and evolution of generative algorithms are constantly expanding.

To address the problem of identifying images from unknown synthetic sources, researchers have recently proposed a variety of open-set and zero-shot approaches. While these methods have demonstrated promising generalization to certain unseen generators, they often rely heavily on optimal threshold selection, which complicates their deployment in practical, real-life scenarios. Moreover, their performance has not consistently extended across the wide range of generative models emerging today.

In this work, we take a different approach by leveraging a fundamental insight from the field of multimedia forensics: the creation process of an image leaves behind microstructures, which can be represented as statistical correlations between adjacent pixel values. Prior work has modeled these forensic microstructures using handcrafted or learned convolutional filters, and then utilized these features for classification purposes. In contrast, our method aims to explicitly capture and leverage these forensic microstructures to create a model that encodes the "forensic state" of each image, allowing the image itself to describe its own unique forensic properties—a concept we refer to as \textbf{forensic self-description}.

Specifically, we first learn to extract forensic microstructures through a self-supervised learning process applied exclusively to real images. These extracted residual fields are then used to construct a forensic self-descriptive model for each image, capturing intrinsic properties of its creation process. Notably, natural images taken by cameras exhibit forensic self-descriptions that are markedly different from those of AI-generated images. By leveraging this insight, our method accurately detects AI-generated images in a zero-shot, unsupervised manner, without relying on prior knowledge of the synthetic generator. Through extensive experimentation, we demonstrate that our approach achieves near-perfect accuracy in distinguishing AI-generated images from real ones, regardless of the real image dataset used for training the extractor.

In addition, we show that our forensic self-descriptions provide a powerful basis for source attribution through unsupervised clustering. This capability allows us to address the challenge of open-set synthetic image detection, enabling both identification of known sources and effective flagging of images from new, unseen synthetic generators. Our results indicate that forensic self-description is a promising direction for tackling the evolving challenge of AI-generated media detection in an open and unsupervised manner.

The main contributions of our paper are as follows:
\begin{enumerate}
	\item We introduce a novel concept of forensic self-description for detecting AI-generated images by modeling the intrinsic forensic microstructures left during image creation.
	\item We propose a self-supervised learning approach to extract forensic microstructures from real images, enabling accurate zero-shot detection of synthetic media without requiring labeled data from generative models.
	\item We demonstrate that our forensic self-description approach effectively clusters real and AI-generated images, supporting both open-set detection and source attribution through unsupervised methods.
	\item  We provide extensive experimental validation, showing that our method achieves near-perfect accuracy in differentiating real images from synthetic ones across a diverse set of generators, highlighting its robustness and practicality for real-world applications.
\end{enumerate}


==> sections/Motivation_v0.tex <==
\subsection{Motivation}

Existing methods for detecting AI-generated images often rely on neural networks trained to recognize forensic microstructures. While effective for known sources, these networks struggle with images from previously unseen generators. This limitation stems from the networks' tendency to learn only the most discriminative microstructural features specific to the training data, leaving out essential forensic details that could generalize to new synthetic sources.

In contrast, our approach constructs a compact, self-contained model of the forensic microstructures for each image, termed a \textbf{forensic self-description}, without requiring labeled data or class-based discriminability. This model captures universal forensic characteristics, enabling accurate performance on several critical tasks: (1) Zero-shot Synthetic Image Detection, (2) Open-set Source Attribution, and (3) Unsupervised Clustering of Image Sources. The following sections detail our method for obtaining and applying these forensic self-descriptions to perform these tasks.



==> sections/ResultsClustering_v0.tex <==
\subsection{Unsupervised Clustering Results}


In this experiment, we assess our model’s ability to cluster images by source in an unsupervised setting, where no labeled data is available. This task is important as it tests the model’s ability to organize images based solely on intrinsic forensic features, crucial for managing unannotated collections in forensic investigations. We report average clustering accuracy, purity, and normalized mutual information (NMI) across different cluster sizes (N, 2N, and 4N), which capture alignment, homogeneity, and information consistency with true labels.

As shown in Tab.~\ref{tab:clustering}, our method achieves the highest scores across all metrics and cluster sizes, with average accuracies of 0.78, 0.80, and 0.83, purity scores of 0.77, 0.81, and 0.85, and NMI scores of 0.69, 0.65, and 0.61, indicating consistent clustering performance across various cluster counts.

Our model’s success is due to its forensic self-description, which captures source-specific microstructures, allowing it to group images by their unique forensic patterns. In contrast, no competing methods are specifically designed for reliable source clustering. Metric-learning methods like FSM, ExifNet, and especially Barni, though trained with Contrastive Learning, rely on embeddings restricted to generators with characteristics seen during training, which limits their unsupervised clustering performance. General-purpose models like CLIP and ResNet-50 also lack the forensic specificity needed for high clustering quality, yielding only moderate accuracy and purity with low NMI.

Notably, UFD performs on par with our method at cluster size = N but falls short at larger cluster sizes. Although UFD is supervised, its objective of separating embeddings by class label aids its clustering performance. Overall, our method’s forensic self-description enables accurate source separation in a fully unsupervised setting, demonstrating both versatility and effectiveness.




==> sections/ResultsClustering_v1.tex <==
\subsection{Unsupervised Clustering Results}


In this experiment, we assessed the ability of forensic self-descriptions to cluster images by source in an unsupervised fashion, where no labeled data is available.
%
We report average clustering accuracy, purity, and normalized mutual information (NMI) across different number of clusters (N, 2N, and 4N), which capture alignment, homogeneity, and information consistency with true labels.

Tab.~\ref{tab:clustering} shows the results of our experiment. These results show that our method achieves the highest scores across all metrics and number of clusters. This strong performance is a result of the self-descriptions fully capturing the forensic microstructures, for which images of a common source naturally cluster together. This is further illustrated in Fig.~\ref{fig:tsne_clustering} where the distribution of the self-descriptions for various sources is presented on a t-SNE plot. From this plot, we observe that the forensic self-descriptions form distinct clusters for each source. In particular, the real images are clearly separated from all synthetic sources, and, among synthetic sources, each generator forms its own tight cluster with well-defined boundaries.

%In contrast, while competing approaches like CLIP and ResNet-50 show moderate performance, their embeddings lack the forensic features that can be used to separate subtle differences between generators in the same family of architectures. Notably, when the number of clusters is equal to the number of sources (N), UFD obtains strong performance, nearly matching our method in accuracy and NMI.

Additionally, in scenarios where the true number of clusters is unknown, a conventional strategy is to cluster with a larger number of clusters and merge based on known information. Under these conditions, our approach shows consistent improvement with increasing number of clusters, while the second-best performer, UFD, experiences declining performance. This trend underscores that our forensic self-descriptions are particularly well-suited for accurate, unsupervised clustering.







==> sections/ResultsOpenSet_v0.tex <==
\subsection{Evaluating Open-Set Source Attribution}


In this experiment, we evaluated the performance of forensic self-descriptions in an open-set setting, where the model must attribute images from known sources to their respective sources while rejecting images from unknown sources.
This task is critical for real-world forensic scenarios, where analysts cannot assume that all test images originate from sources observed during training.
The model, therefore, needs to identify images from unknown sources at test time to avoid misattribution.

We present the results in Table~\ref{tab:open_set}.
Our method demonstrates strong performance across both closed-set and open-set tasks.
Specifically, we achieve the highest performance in rejecting images from unknown sources, with an AU-CRR of 0.933—approximately 7\% higher than the best competitor, Fang et al., and 18\% higher than RepMix.
This performance gain is due to our self-description mechanism, which is finely tuned to capture each source's unique forensic traces, enabling the GMMs to accurately model source-specific image distributions and effectively reject unknown images.
In contrast, Fang et al. and RepMix employ a common embedding space for all known sources, aiming to separate each source from the rest, but this approach may struggle to separate unknown sources effectively, especially when unknown and known sources share similar forensic characteristics.

Our method also achieves competitive closed-set source attribution accuracy, with an accuracy of 0.964, only 0.02 below the best competitor, Fang et al.
This gap arises because fully supervised methods like Fang et al. explicitly optimize the embedding space for source separation, while our self-supervised method relies solely on the accuracy of self-descriptions, rather than explicitly optimizing for closed-set attribution.

Lastly, we achieve an AU-OSCR of 0.913, which is approximately 6\% higher than the best competitor, Fang et al., and 17\% above RepMix, the second-best competitor.
These results highlight our method’s superior balance between closed-set and open-set performance, demonstrating that utilizing self-descriptions for source attribution is highly effective in real-world forensic scenarios.

%In this experiment, we evaluated the performance of forensic self-descriptions in an open-set setting, 
%where the model must attribute images from known sources to their respective sources,
%while rejecting images from unknown sources.
%This task is critical for real-world forensic scenarios, 
%where forensic analysts cannot assume that all test images come from sources observed during training.
%Here, the model needs to identify images from unknown sources at test time to avoid misattribution.
%
%We present the results of this experiment in Table~\ref{tab:open_set}.
%The results demonstrate the strong performance of our method in both closed-set and open-set tasks.
%Specifically, we achieve the best performance in rejecting images from unknown sources with an AU-CRR of 0.933, being 
%approximately 7\% higher than the best competitor, Fang et al., and 18\% higher than RepMix. We attribute this performance 
%gain to the self-description mechanism, which is highly tuned to each source's unique forensic traces, enabling the GMMs to
%accurately model the source-specific image distributions. Therefore, our method can effectively reject images from unknown sources. 
%In contrast, Fang et al. and RepMix learn a common embedding space for all known sources with the goal of 
%separating each known source from the rest. This does not guaranty to produce an embedding space in which the 
%unknown sources are well separated from the known sources 
%especially when the unknown and known sources show similar forensic characteristics.
%
%
%Our method also achieves a competitive closed-set source attribution accuracy of 0.964 which only falls behind the best competitor, 
%Fang et al., by 0.02. This gap is because fully supervised methods \eg Fang et al. explicitly optimize
%their embedding space to separate known sources,
%while our method does not explicitly optimize for this task and only relies on the highly accuarate self-descriptions which are 
%learned in a self-supervised manner. 
%
%
%Lastly, we achieve an AU-OSCR of 0.913, approximately 6\% higher than the best competitor, Fang et al., and 17\% above RepMix, the second best competitor.
%This result clearly demonstrates the superior performance of our method in balancing closed-set and open-set performance and proves 
%utilizing self-descriptions for source attribution is highly effective in real-world forensic scenarios.

% Our method outperforms all competing methods in terms of AU-CRR and AU-OSCR, and achieves competitive performance in 
% closed-set source attribution. These results demonstrate the top performance of our method in rejecting images from unknown sources,
% while maintaining high accuracy in attributing images from known sources. Additionally, according to the AU-OSCR metric, our method
% achieves the best balance between closed-set and open-set performance, outperforming all competing methods.

% Comparatively, our method's AU-CRR is approximately 7\% higher than the best competitor, Fang et al., and 30\% higher than POSE.


% However, the most salient finding is our method's strong ability to reject images from unknown sources, 
% a key open-set challenge.
% Our method achieves an AU-CRR of 0.933, which substantially outperforms all competing methods. Specifically,
% our AU-CRR is approximately 7\% higher than the best competitor, Fang et al., and 30\% higher than POSE, which 
% are both explicitly designed for open-set synthetic image source attribution.

% , 
% including Fang et al. (0.856), Abady et al. (0.640), and RepMix (0.746).
% Notably, our method surpasses Fang et al. by a margin of 7\% in AU-CRR, 
% underscoring the difficulty of open-set source rejection during testing, 
% even for methods explicitly designed for open-set attribution.

% Lastly, considering the AU-OSCR metric, which balances closed-set and open-set performance, 
% our approach clearly outperforms all competing methods.
% We achieve an AU-OSCR of 0.913, approximately 6\% higher than the best competitor, Fang et al., and 17\% above RepMix.
% This performance gain is because unlike the competing methods our method does not rely on any known synthetic images 
% to learn the image representations.
% Reliance on known synthetic images can lead drop of performance especially in open-set scenarios where the unknown data distribution 
% can be very different from the known data distribution.

==> sections/ResultsOpenSet_v1.tex <==
\subsection{Open-Set Source Attribution Results}


In this experiment, we evaluate our model’s ability to attribute synthetic images to their source in an open-set setting, where it must identify images from known sources while rejecting those from unknown sources. We report average accuracy for known classes, AU-CRR, and AU-OSCR to capture both source attribution and unknown-source rejection.



From Tab.~\ref{tab:open_set}, we observe that our method achieves the highest AU-CRR (0.933) and AU-OSCR (0.913) and near-best accuracy (0.964), third only to Fang’s 0.988 and RepMix's 0.982. These results demonstrate our model’s reliability in rejecting unknown sources while maintaining high accuracy in known-source attribution.


Our model’s success is due to its detailed forensic self-descriptions, which capture distinct microstructural patterns for each source, enhancing attribution even when encountering new generators. In contrast, transferable embedding methods like CLIP and ResNet-50 show low accuracy (0.570 and 0.538) and poor rejection scores, as their generic embeddings lack the forensic specificity for source attribution. Supervised models such as RepMix perform well on known sources (0.982 accuracy) but have a lower AU-CRR (0.746), reflecting limited open-set adaptability. Similarly, metric-learning methods FSM and ExifNet struggle, with ExifNet showing particularly low accuracy (0.186) due to its reliance on forensic features that do not generalize well to synthetic images.


Notably, open-set methods like POSE and Barni achieve moderate accuracies but fall short in AU-CRR and AU-OSCR compared to our model, as they rely on embedding spaces learned during training to generalize to new generators. However, it is challenging to preemptively design embeddings for unknown generators. Our method, by contrast, builds unique forensic features per source, avoiding reliance on pre-trained embeddings and thus excelling in both source attribution and unknown-source rejection.





==> sections/ResultsOpenSet_v2.tex <==
\subsection{Open-Set Source Attribution Results}


In this experiment, we evaluated the ability to attribute synthetic images to their source in an open-set fashion using forensic self-descriptions. Here, methods must identify images from known sources while rejecting those from unknown sources. We report average accuracy to show attribution performance among known sources, AU-CRR to show the performance identifying if an image comes from known or unknown sources, and AU-OSCR to capture both aspects.


Tab.~\ref{tab:open_set} shows the results of this experiment. These results show that our method achieves the highest AU-CRR (0.933) and AU-OSCR (0.913). We also obtained near-best accuracy (0.964), behind Fang’s 0.988 and RepMix's 0.982. These results demonstrate that forensic self-descriptions can be used to both accurately attribute an image to its source, and determine when an image was generated using a new or unknown source.


Our strong results is due to the fact that forensic self-descriptions capture distinct microstructural patterns for each source, enhancing attribution even when encountering new generators.
%
In contrast, while supervised methods like RepMix perform well on known sources (0.982 accuracy), they obtain a lower AU-CRR (0.746). This shows that their learned features during training do not transfer well to new sources.

Additionally, dedicated open-set methods like POSE and Barni achieve moderate accuracies but fall short in AU-CRR and AU-OSCR compared to our model, as they rely on embedding spaces learned during training to generalize to new generators. However, it is challenging to preemptively learn embeddings for unknown generators. Notably, Fang obtained strong performance accross all three metrics but our method still outperform Fang on AU-CRR and AU-OSCR. This show that by avoiding reliance on explicit supervision using labels, forensic self-descriptions can fully capture the forensic microstructures in any image to enable accurate open-set attribution of image sources.





==> sections/ResultsOpenSet_v3.tex <==
\subsection{Open-Set Source Attribution Results}


In this experiment, we evaluated the ability to attribute synthetic images to their source in an open-set fashion using forensic self-descriptions.
Here, methods must accuratelt attribute an image to its source while also determining if it originates from an unknown source.
We report average accuracy for known-source attribution, AU-CRR to assess identification of known versus unknown sources, and AU-OSCR to capture both aspects.


Tab.~\ref{tab:open_set} shows the results of this experiment. These results show that our method achieves the highest AU-CRR (0.933) and AU-OSCR (0.913). We also obtained near-best known source accuracy (0.964), behind Fang’s 0.988 and RepMix's 0.982.
These results indicate that forensic self-descriptions allow both accurate attribution among known sources and reliable identification of unknown sources.


Our strong results is due to the fact that forensic self-descriptions capture distinct microstructural patterns for each source, enhancing attribution even when encountering new generators.
%
In contrast, while supervised methods like RepMix perform well on known sources (0.982 accuracy), their lower AU-CRR (0.746) reflects limited transferability to unknown sources.



Additionally, dedicated open-set methods like POSE and Abady achieve moderate known source accuracies but fall short in AU-CRR and AU-OSCR compared to our approach, as they rely on embedding spaces learned during training to generalize to new generators. However, it is challenging to preemptively learn embeddings for unknown generators. Notably, while Fang performs well across all metrics, our method still surpasses Fang on AU-CRR and AU-OSCR.
This show that by learning self-descriptions that capture all aspects of the forensic microstructures and not just those useful for discriminating between known sources during training, we can peform accurate open-set attribution of image sources.





==> sections/ResultsZeroShot_v0.tex <==
\subsection{Evaluating Zero-Shot Detection}

The goal of this experiment is to evaluate our approach for zero-shot synthetic image detection
where the task is to identify AI-generated images from real images without 
any prior training on the specific generative model.
This task is crucial in real-world applications, 
as the rapid advancement of synthetic image generation makes it 
impractical to assume that all potential synthetic sources will be known during training.
Thus, a robust model must generalize to new, 
unseen synthetic sources even the ones that are substantially different from the ones seen during training.
% without prior exposure to their specific characteristics.

We provide the results of our zero-shot detection experiment in Table~\ref{tab:zero_shot}. Each column in the table shows
the average AUC of all the pairs of synthetic sources with the corresponding real dataset. The overall 
average AUC of all the pairs is
provided in the last column.
The results show that by relying on forensic self-descriptions, our method consistently achieves 
the best performance in zero-shot synthetic image detection accross all real datasets. The overall average AUC of our method is 0.96,
which is approximately 0.04 higher than the best competitor, NPR, and 0.13 higher than the second best competitor, PatchFor. 
This strong performance is because our method is a completely unsupervised and does not need any synthetic images. This is an
advantage over the supervised methods, as they face challenges in generalizing to new synthetic generators that were not seen
during training.
Therefore, it can reliably model the forensic microstructures of real images

==> sections/ResultsZeroShot_v1.tex <==
\subsection{Zero-Shot Detection Results}


In this experiment, we evaluate our model’s ability to detect synthetic images from unknown generators in a zero-shot setting, a critical test of robustness and generalizability to unseen synthetic sources for practical forensic applications. We report the average AUC across all real-vs-synthetic dataset pairs, which captures threshold-independent performance in distinguishing real from synthetic images.



From Tab.~\ref{tab:zero_shot}, we observe that our method achieves the highest performance, with an overall average AUC of 0.960 across datasets, surpassing all other competing approaches. Specifically, our model attains AUCs of 0.968, 0.960, 0.941, and 0.971 on COCO17, ImageNet-1k, ImageNet-22k, and MIDB, respectively, consistently leading across datasets. The next-best model, NPR, has an average AUC of 0.926, with its highest AUC on MIDB (0.957), which remains lower than our method.


Our method’s superior results are due to its reliance on forensic microstructures, which show distinctive patterns between real and synthetic images. In contrast, methods like CnnDet, PatchFor, LGrad, and UFD suffer from limited transferability of their embedding spaces, making them less adaptable to new generators. Zero-shot methods such as ZED, DE-FAKE, and Aeroblade perform well with certain generators—ZED on DALLE's, DE-FAKE on SD 3.0, and Aeroblade on MJ's—but their overall performance is lower. This inconsistency arises from their focus on generalized, microstructure-less features that, in practice, do not reliably generalize across diverse generative methods. By capturing forensic microstructures, which are inherently distinct between real and synthetic images, our method ensures robust and reliable zero-shot detection across a wide range of generators.








==> sections/ResultsZeroShot_v2.tex <==
\subsection{Zero-Shot Detection Results}


In this experiment, we evaluated our forensic self-description’s ability to detect synthetic images from unknown generators in a zero-shot setting, a critical test of robustness and generalizability to unseen synthetic sources for practical forensic applications. To do this, we report the average AUC across all 24 real-vs-synthetic dataset pairs per real source. The full results is presented in the supplemental materials.

We present the results of this experiment in Tab.~\ref{tab:zero_shot}. These results show that our method achieves the highest performance, with an overall average AUC of 0.960 across datasets, consistently surpassing all other competing approaches. Specifically, our model attains AUCs of 0.968 on COCO17, 0.960 on ImageNet-1k, 0.941 on ImageNet-22k, and 0.971 on MIDB. The next-best model, NPR, has an average AUC of 0.926, with its highest AUC on MIDB of 0.957, which remains lower than our method.

Our method's strong zero-shot detection performance is due to the use of forensic self-descriptions, which show distinctive patterns between real and synthetic images. This is illustrated further in Fig.~\ref{fig:self_desc_viz}.
%
In contrast, methods like CnnDet, PatchFor, LGrad, and UFD suffer from limited transferability of their embedding spaces, making them less adaptable to new generators.

Furthermore, as detailed in the supplemental materials, zero-shot methods such as ZED, DE-FAKE, and Aeroblade show good performance with certain generators—ZED with DALLE, DE-FAKE with SD 3.0, and Aeroblade with MJ—but their overall results are inconsistent. This inconsistency likely arises because the generalized features these methods rely on lack the nuance to reliably capture diverse generative methods. By contrast, our method robustly captures forensic microstructures, which are inherently distinct between real and synthetic images, ensuring reliable zero-shot detection across a broad range of generators.




==> sections/ResultsZeroShot_v3.tex <==
\subsection{Zero-Shot Detection Results}


In this experiment, we evaluated our forensic self-description’s ability to detect synthetic images in a zero-shot setting, a critical test of generalizability to unseen synthetic sources for practical forensic applications. To do this, we report the average AUC across all 24 real-vs-synthetic dataset pairs per real source. The full results is shown in the supplemental materials.

We present the results of this experiment in Tab.~\ref{tab:zero_shot}. These results show that our method achieves the highest zero-shot detection performance, with an overall average AUC of 0.960 across all datasets. In contrast, supervised methods like CnnDet, PatchFor, LGrad, and UFD obtain lower performance overall. This is because the features they learned during training do not transfer well to new generators.

Additionally, while zero-shot methods such as ZED, DE-FAKE, and Aeroblade show strong performance on some generators, they struggle on other generators. As can be seen from the results in the supplemental materials, ZED struggled with ProGAN (0.462) and Firefly (0.563), DE-FAKE with StyleGAN 3 (0.590), and Aeroblade with BigGAN (0.425) and DALLE 2 (0.596). In contrast, our method displays consistently strong performance, irrespective of the generator or real source. This is because our forensic self-descriptions fully captures the forensic microstructures, which are inherently distinct between real and synthetic images, ensuring reliable zero-shot detection across a broad range of generators.




==> tables/Clustering_v0.tex <==

\begin{table*}
    \centering
    \label{tab:clustering}
    \caption{Clustering performance comparisons with various techniques.}
    \resizebox{0.70\linewidth}{!}{
        \begin{tblr}{
            width = \linewidth,
            colspec = {|m{24mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|m{9mm}|},
            row{2} = {c},
            cell{1}{1} = {r=2}{},
            cell{1}{2} = {c=3}{0.2\linewidth,c},
            cell{1}{5} = {c=3}{0.2\linewidth,c},
            cell{1}{8} = {c=3}{0.2\linewidth,c},
            cell{1}{11} = {c=3}{0.198\linewidth,c},
            cell{3-12}{2-13} = {c},
            vlines,
            vline{2,5,8,11} = {2}{solid,black},
            vline{2,5,8,11} = {2}{2}{solid,black},
            vline{2,5,8,11} = {1-12}{solid,black},
            vline{2,5,8,11} = {2}{1-12}{solid,black},
            hline{1,3,5,8,12-13} = {-}{},
            hline{2} = {2-13}{},
        }
        \textbf{ Method} & \textbf{\# Clusters = N} &  &  & \textbf{\# Clusters = 2N } &  &  & \textbf{\# Clusters = 4N } &  &  & \textbf{\# Clusters = 8N } &  & \\
        & {\textbf{Avg.}\\\textbf{Acc.}} & \textbf{Purity} & \textbf{NMI} & {\textbf{Avg.}\\\textbf{Acc.}} & \textbf{Purity} & \textbf{NMI} & {\textbf{Avg.}\\\textbf{Acc.}} & \textbf{Purity} & \textbf{NMI} & {\textbf{Avg.}\\\textbf{Acc.}} & \textbf{Purity} & \textbf{NMI}\\
        CLIP~\citethis & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --\\
        ResNet-50~\citethis & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --\\
        FSM~\citethis & 0.16 & 0.16 & 0.01 & 0.18 & 0.18 & 0.02 & 0.20 & 0.20 & 0.03 & 0.44 & 0.22 & 0.04\\
        ExifNet~\citethis & 0.21 & 0.22 & 0.06 & 0.24 & 0.26 & 0.08 & 0.32 & 0.28 & 0.09 & 0.45 & 0.27 & 0.08\\
        Barni~\citethis & 0.18 & 0.18 & 0.01 & 0.19 & 0.19 & 0.03 & 0.21 & 0.21 & 0.03 & 0.22 & 0.22 & 0.03\\
        CnnDet~\citethis & 0.47 & 0.36 & 0.28 & 0.49 & 0.38 & 0.27 & 0.52 & 0.42 & 0.26 & 0.55 & 0.46 & 0.26\\
        NPR~\citethis & 0.46 & 0.39 & 0.34 & 0.57 & 0.48 & 0.33 & 0.63 & 0.51 & 0.32 & 0.64 & 0.54 & 0.31\\ 
        DE-FAKE~\citethis & 0.32 & 0.25 & 0.16 & 0.24 & 0.25 & 0.14 & 0.22 & 0.25 & 0.12 & 0.22 & 0.25 & 0.12\\
        UFD~\citethis & 0.78 & 0.71 & 0.68 & 0.67 & 0.69 & 0.55 & 0.71 & 0.72 & 0.50 & 0.70 & 0.75 & 0.47\\
        \textbf{Ours} & \textbf{0.78} & \textbf{0.77} & \textbf{0.69} & \textbf{0.80} & \textbf{0.81} & \textbf{0.65} & \textbf{0.83} & \textbf{0.85} & \textbf{0.61} & \textbf{0.86} & \textbf{0.87} & \textbf{0.58}
        \end{tblr}
    }
\end{table*}

==> tables/ZeroShot_v0.tex <==

\begin{table}
    \centering
    
    \caption{\label{tab:zero_shot}Average zero-shot synthetic image detection performance over all pairs of a real dataset vs each synthetic generator source. Metrics are reported using AUC.}
    \resizebox{1.0\linewidth}{!}{
        \begin{tblr}{
            width = \linewidth,
            colspec = {|m{24mm}|m{14mm}|m{13mm}|m{13mm}|m{12mm}|m{12mm}|},
            row{2} = {c},
            column{6} = {c},
            cell{1}{1} = {r=2}{},
            cell{1}{2} = {c=4}{0.80\linewidth,c},
            cell{1}{6} = {r=2}{},
            cell{3-11}{2-5} = {c},
            vlines,
            hline{1,3,11-12} = {-}{},
            hline{2} = {2-5}{},
        }
        \textbf{Method} & \textbf{Average AUC of all pairs w.r.t a real dataset} &  &  &  & \textbf{Average}\\
        & \textbf{COCO17} & \textbf{IN-1k} & \textbf{IN-22k} & \textbf{MIDB} & \\
        CnnDet~\cite{CNNDet} & 0.756 & 0.714 & 0.733 & 0.683 & 0.722\\
        PatchFor~\cite{PatchFor} & 0.833 & 0.823 & 0.845 & 0.790 & 0.823\\
        UFD~\cite{UFD} & 0.903 & 0.862 & 0.815 & 0.612 & 0.798\\
        LGrad~\cite{LGrad} & 0.819 & 0.770 & 0.866 & 0.824 & 0.820\\
        DE-FAKE~\cite{DE-Fake} & 0.765 & 0.749 & 0.617 & 0.791 & 0.731\\
        Aeroblade~\cite{Aeroblade} & 0.728 & 0.741 & 0.582 & 0.646 & 0.674\\
        ZED~\cite{Zed} & 0.751 & 0.676 & 0.716 & 0.747 & 0.723\\
        NPR~\cite{NPR} & 0.945 & 0.900 & 0.900 & 0.957 & 0.926\\
        \textbf{Ours} & \textbf{0.968} & \textbf{0.960} & \textbf{0.941} & \textbf{0.971} & \textbf{0.960}
        \end{tblr}
    }
\end{table}
